An Open-Ended Approach to Understanding Local, Emergent Conservation Laws in Biological Evolution

While fields like Artificial Life have made huge strides in quantifying the mechanisms that distinguish living systems from non-living ones, particular mechanisms remain difficult to reproduce in silico. Known as open-endedness, we've been successful in finding mechanisms that generate new states, but have been less successful in finding mechanisms that generate new rules. Here, we weigh whether or not analyzing the effects of internal and external system constraints on a system's dynamics would be a fruitful avenue to understanding open-endedness. We discuss the connection between physical constraints and the ways that the system can physically reach possible states while those constraints are present. It seems that the physical constraints that define biological objects (and dynamics) are maintained by dynamics that occur from within the system. This is in opposition to current modeling approaches where system constraints are maintained externally. We suggest that constraints can be characterized as variables whose values are either completely conserved, quasi-conserved, or conditionally conserved. Regardless of whether or not a constrained variable is a part of the biological object or present in the object's environment, we discuss how the accessible system states under that constraint can lead to local, emergent conservation laws (rules), with examples. Finally, we discuss the possible benefits of formally understanding how system constraints that emerge from within a system lead to system dynamics that can be characterized as new, emergent rules -- particularly for artificial intelligence, hybrid life, embodiment, astrobiology, and more. Understanding how new, local rules might emerge from within the system is crucial for understanding how open-ended systems continually discover new update rules, in addition to continually discovering new states.

==> notes.tex <==

----------------- MATH APPROACHES NOTES

The emergence of slow and fast degrees of freedom depends on the value of that variable. If the entropy of such a marginalized process goes up, then some important, underlying processes was elft out of the ``good'' description of the system. This introduces uncertainty into the marginalized system's description.

Origin of life and major evolutionary transitions for ALIFE. How do we program them?

There are two approaches to understanding this from a computational perspective. The first is to consider a type of object, and then explore the dynamics of that type of object as it interacts with a kind of environment. Depending on the environment and the interaction rules, the objects can change their physical or behavioral characteristics. The second approach involves considering the dynamics of the system as a whole and applying some type of object-detection method to identify potential objects with life-like characteristics. In both of these approaches, the programmer needs to have some idea of an object to begin with. (Adjacent possible, Taylor, Montevil papers)

Defining an object in living systems is notoriously difficult because it can often appear up to an external observer to detect or choose a defining set of variables. This can be problematic for ALife because real, living systems often define objects from within the dynamics of the system. In addition, major evolutionary transitions in biology seem to be focused on defining new kinds of objects that can perform kinds of computations. (Ackerman paper)

It has been suggested that one of the first major transitions for the origin of life is the ability for "objects" to self-maintain (papers for autocatalysis). Why is this important for ALife? Because if ALife wants to achieve life-like evolution that can run on its own without an external user programming major transitions by hand, then it is important to understand how new objects first get created. In other words, how does a possible object become a "meaningful" object (one that maintains its state over time) through the dynamics of the whole system? (Wong and Bartlett papers)

(Can also talk about other essential functions in bio from Wong paper, major evolutionary transitions papers)

In this paper, we explore a graph-theoretic method that considers all possible objects, but identifies particular objects that have a particular type of relationship between their own states and the states of the rest of the environment (or part of the environment, or second object?). While there are many kinds of possible relationships, we focus on the kind of relationship that keeps the objects in a state (or subset of states), given states of the environment. This is done by considering the dynamics of the whole system, the dynamics of that object, and the dynamics of the environment simultaneously. 

The goal is to characterize aspects of the system topology that allow this type of relationship to happen. Are there characteristics of the system states or the object states that allow this relationship between the object and environment to remain present?




First, we start with a system state space topology. The goal is to find objects that have that relationship between its own states and the environment's states. Then, to identify which system constraints (variables with fixed values) contribute to this relationship (or not). The reason for considering the constraints is because the points made in Taylor and Montevil. We support the view that a system can be characterized by the state space of every possible state, even if every possible states are never physically realized. Biological systems are physically realizing some of those states by exploring sub-regions of the topology.

Perturbation analysis: Consider the original graph. First, select an arbitrary object. Then, select a region of the graph where one variable remains as a single fixed value. Then, compare the region of the graph where this variable is the opposite value. Compare the topology of these two regions.

Need: A metric that characterizes whether or not the relationship between object states and environment states looks like the regulation/autocatalysis/homeostatis function from Wong paper. Scale from 0-1? 0 is the relationship has no correlation, basically the state of the object is random, given the state of the environment. 1 is there is a many-to-one relationship between environment states and object states.

Also need: A metric between a system constraint and difference in subgraph topologies.

Main result figure: A plot between the second metric vs the first metric. One line color per graph type?

Careful: Need to make this different from sensing. Maybe sensing is a stronger form than the first function. Sensing has the added property that the relationship is object states are a coarse-graining of environment states (multiple many-to-one mappings). But regulation is many-to-less states.

Eric Smith's paper: intrinsic and extrinsic thermodynamics. If you marginalize over the environment variables, what do you get? The intrinsic part is the system and the extrinsic system. Given the generator of the system, what is the generator for the system given some marginalized variables? <-- is the motivation --> So then how do we translate that into a graph theoretic formalism? 

How do users pick variables to coarse grain and to create labels? Finding tools means creating labels. Is it possible? How can we connect this to Eric's paper?

Tools as constraint: Some variable defined over the nodes, and any links conencting to that variable are turned off. These variables are the long-term dynamics, the constraints. How do agents find those constraints? Just thinking about constraints and not sys/environbment, in all the ways we can partition the components of the labels in a certain way such that the reduced stochastic matrix to find a separation of timescales. How does it relate ton ALIFE? Find an algorithm to do that? Check all different partiiotns and their spectrums, then look at qualities. Matricx finding problem. Then, finding these partitions in real life. Once you have this separation of time scales, in the shoprter one (everything but the constraints). Then finding a ratcheting effect? This is what Nich means about the labels. WHICH PARTITION CORRESPONDS TO A CONSTRAINT? 

Propose: Such a partition is a constraint where the EVs are easily separated. Would need to go over all different possibilities to check partitions. But then you can take T' and further re-partition it. 

Conservation law: The time derivative of it is zero. Then might have things like quasi-conserved, slow or difficult to change. Like Nitrogen fixtion. Conditionally conserved: more speciic, when some system is in some set of variables, then another things time derivative will be zero, but if changed then the other thing will not be zero. So the emergence of slow and fast degrees of freedom depends on this variable. So, its not a function of the dynamiocs you get when you marginaize. Measure the entropy generation, then if it goes up then you deleted some physics. Then its extra uncertainty. 

Write these as propdcuts of 2 markov processes, and all the fast time stuff is in one and the sow is in the other. Can you find a decomposition that does something nice with the separation of time scales? Run over all the partitions for some particular case? 

Taking existing constraints, ones that are applied externally, but the math is done looking at the system evolves under those constraints (usual approach)
vs
What does it look like when the system creates a conditionally conserved variable? Vs when its conversed vs when it doesn't. Bifurcations? Finding ways to find them. And then can we find a fractal/ratcheting process.

Note about using graph formalism:
State graph framework to think about the world vs what does it look like when a system constrains itself. Consequences of the choice of using graph: Graph dervied from looking at variables to follow? Really talking about microstates of the system? Graph of the universe? We have no chopice but to start with a choice. Writing the labels and the edges in the graph is already coarse-graining, even if its fine-grained. 




----------------- MATH MODEL AND METHODS

\section{Mathematical model of conserved laws}

\subsection{Definitions}

Set of states or state space $S$.

A probability vector P over the state space is an $S$ vector that
satisfies
\begin{align*}
\sum_{n\in S}P_{n} & =1.\\
P_{n} & \geq0.
\end{align*}

A probability vector will be said to lie in the unit simplex. 

A time-dependent probability vector is given by $P(t)$, where $t$
is a discrete index.

A stochastic process is given by $S\times S$ matrix $\Lambda$, called
the stochastic matrix, such that
\[
P_{n}(t+1)=\sum_{m}\Lambda_{nm}P_{m}(t),
\]

or 
\begin{equation}
P(t+1)=\Lambda P(t).\label{eq:stoch_process}
\end{equation}

A stochastic matrix satisfies
\begin{equation}
\sum_{n}\Lambda_{nm}=1\hspace{1em}\forall m\in S.\label{eq:stoch_matrix}
\end{equation}


\subsection{Slow time scales}

Thus far in our meetings, we have discussed considering the spectrum
of the stochastic matrix and obtaining different time scales. Consider the set of normalized eigenvectors $B$ such that for each $b\in B,$

\[
\Lambda b=\lambda_{b}b,
\]

where 
\[
1\leq\lambda_{b}\leq\lambda_{\text{\text{thresh.}},}
\]

where $\lambda_{\text{thresh.}}$ is some threshold defining the slow
time scale. 

The vectors in the set B yield a subspace of the unit simplex where
the dynamical system evolves slowly. Notice that the stationary distribution corresponding to $\lambda_{b}=1$ also lies in the subspace. Thus
the dynamics of the probability vector under the stochastic matrix
can be visualized as slowly changing and approaching this stationary
distribution.


\subsection{Conservation laws and conserved quantities}

An $S$ vector $O$ is a conservation law if 
\[
\sum_{n}O_{n}P_{n}(t)=\sum_{m}O_{m}P_{m}(t+1)=o
\]

and $o$ is the conserved quantity. Notice that although the probability
vector is evolving under the stochastic matrix, the conservation law
provides a weighting over the states such the value of the weighted
sum (weighted by the conservation law) of the probability vector over
the state space is constant. 

Equivalently, we write this as 
\[
O^{T}P(t)=O^{T}P(t+1).
\]

Using the stochastic matrix from \ref{eq:stoch_process}, we get

\[
O^{T}P(t)=O^{T}\Lambda P(t),
\]

or 
\[
O^{T}(\Lambda-I)P(t)=0
\]

for any probability vector $P(t).$ A stronger condition is that matrix
$M$ such that

\[
M=(\Lambda-I),
\]

has a left zero-eigenvector, or a left eigenvector with $0$ eigenvalue.
It is stronger as the restriction on $P(t)$ to be a probability vector
is lifted. 

The condition for a conservation law is 

\begin{equation}
\exists O\neq\textbf{0}\hspace{1em}\text{s.t.}\hspace{1em}O^{T}M=\textbf{0}.\label{eq:conservation_law}
\end{equation}


\paragraph*{Example}

Define
\[
e=[1,1,\ldots,1]^{T}.
\]

Using \ref{eq:stoch_matrix}, we get 

\[
e^{T}(\Lambda-1)=\textbf{0}.
\]

Thus $e$ is a conservation law, corresponding to conservation of
probability, and the total probability is a conserved quantity. It
is set equal to one by the initial conditions. 

\subsection{Conditional conservation laws}

There are several ways in which one can generalize Eq. \ref{eq:conservation_law}. 

A conditional conservation law can be seen as one that conserves the
quantity in a subset of states. 

Let $U\subset S$. If there is a vector $O_{U}$ such that

\begin{equation}
O_{U}^{T}(\Lambda-I)\bigg|_{U}=\boldsymbol{0}.\label{eq:cond_conservation}
\end{equation}

Finding such an $O_{U}$ is simple. First, notice that there is a
subspace of vector which satisfy this property. The basis vectors
of this subspace can be found as follows.
\begin{enumerate}
\item Find the (pseudo) inverse of $(\Lambda-I)^{T}$. Notice that the $i^{\text{th}}$
column of the inverse maps to the unit vector with $1$ on the $i^{\text{th}}$index
and $0$ elsewhere. 
\item The basis vectors are given by all the columns of the inverse that
correspond to every element in the complement of the set U in S. It
can be see easily that all of these vectors satisfy \ref{eq:cond_conservation}.
\end{enumerate}


\section{Methods}

\begin{itemize}
    \item Compute eigen system
    \item The first easy choice for SCL/almost-SCl/Conditional-SCL can be among the left-eigenvectors of matrix $M=\Lambda-I$ defined in the section on math model of SCL
    \item Set an $epsilon$ such that every eigenvector which eigenvalue's norm is bellow $epsilon$ is considered an SCL
    \item Verify that $\mathbf{1}^T$ is an SCL as the definition implies
    \item Check if there are conditional SCL among the almost-SCL (i.e. components of the eigenvector are identically 0
    \item To which states the conditions apply? relatively to the context of the system, what information does it give us?
    \item Analyze how well a conditional or almost-SCL of interest conserves the quantities under the repeated application of the transition matrix:
    \begin{itemize}
        \item Compute $O^k.(L^{k+1}-I)-O^k.(L^{k}-I)=O^k.L^{k}.M$
        \item The components of the resulting vector depending on $k$ indicate the rates at which the application of $\Lambda$ is disturbing the conservation
        \item Plot the curves for each 
    \end{itemize}
    \item Analyze the structure of the probability vector $p^*$ for which an almost-SCL can be a perfect SCL ($O^k.(L^k-I).p=\mathbf{0}$ -> the $p$ that are orthogonal to $O^k.(L^k-I)$)
    \item Can do a perturbation analysis around this $p^*$? ({\color{blue} [Eliott] -- I don't have results for that yet, so it's a bit late})
\end{itemize}


{\textbf{Initial notes}:
Look at all these different types of graphs. 
Do spectral analysis to look at the eigenvalues, set the small ones to zero and then rebuild the graphs.
Writing the process as a produce of two processes (setting them to zero). If all of the slow stuff were constant instead of slow. The EValues tell you how fast or slow, the speed is 1/1-EV, which is the characteristic timescale where it decays. Conceptually, is to find the separation of scales and say that things on one side of that separation as if the things on the other side are constant. Factorizing the markov process means setting these "slow values" to 0. Basically factorizing the slow processes of a markov process from a fast one. Then can solve them separately for things like phase transition problems in physics.}

\section{Results}
{\color{blue} [Eliott] -- I suggest using Markov chains that are close to the epidemiological models SIS, SIR, SIRS. But do we want to explicitly say that they are such models and to ground them in the context of epidemiology? I don't know in this conference but my knowledge of the state-of-the-art in this area is rusty and 5 years old so might get attacked by someone saying that "this has already been done" even if we use this context only for illustrating purposes. \\Also, this context is not very ALife...}

\paragraph{Example SIS-like} 2-states loop with self-transitions; Identify the conservation law that promotes staying in the S state.

\paragraph{Example SIR-like } 3-states linear with self-transitions;  Identify the conservation law that promotes staying in the R state. Discuss in context how good the SCL is to avoid getting infected (transition S to I). How can we structure the probability distribution p to help the SCL doing it's job of keeping stuffs in R? In SIR, it should be simply $[0,0,1]$. Trivial result in this case, but what about larger model with multiple treatments, vaccines, viral strains?

\paragraph{Example SIRT multiclass} {\color{blue} (ref for the type of model even if it's ODE-based https://royalsocietypublishing.org/doi/10.1098/rsif.2020.0105)} The value of our analysis method lies in big state universes. Can we identify SCL in epidemiological models accounting for multiple treatments and microbe strains? This is relevant for the optimization of treatments strategy to mitigate acquisition of multi-drug resistances. Can we find SCL that conditionally weakens the multi-drug resistant strains.

\paragraph{More general considerations} Show that for different transition matrices, the SCL are obviously different and that almots-SCL in one situation are not in the other. If the transition matrices are set per environment then, and a conditional SCL represents how a population fits in a subset of the universe, conditional-SCLs can be used to compare the "fitness" of systems in different environments.
